PAIR-Diffusion: A Comprehensive Multimodal Object-Level Image Editor

Generative image editing has recently witnessed extremely fast-paced growth. Some works use high-level conditioning such as text, while others use low-level conditioning. Nevertheless, most of them lack fine-grained control over the properties of the different objects present in the image, i.e. object-level image editing. In this work, we tackle the task by perceiving the images as an amalgamation of various objects and aim to control the properties of each object in a fine-grained manner. Out of these properties, we identify structure and appearance as the most intuitive to understand and useful for editing purposes. We propose PAIR Diffusion, a generic framework that can enable a diffusion model to control the structure and appearance properties of each object in the image. We show that having control over the properties of each object in an image leads to comprehensive editing capabilities. Our framework allows for various object-level editing operations on real images such as reference image-based appearance editing, free-form shape editing, adding objects, and variations. Thanks to our design, we do not require any inversion step. Additionally, we propose multimodal classifier-free guidance which enables editing images using both reference images and text when using our approach with foundational diffusion models. We validate the above claims by extensively evaluating our framework on both unconditional and foundational diffusion models. Please refer to https://vidit98.github.io/publication/conference-paper/pair_diff.html for code and model release.

==> bib_bak.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@article{ling2021editgan,
  title={Editgan: High-precision semantic image editing},
  author={Ling, Huan and Kreis, Karsten and Li, Daiqing and Kim, Seung Wook and Torralba, Antonio and Fidler, Sanja},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={16331--16345},
  year={2021}
}


@misc{Authors14,
 author = {Full Author Name},
 title = {The Frobnicatable Foo Filter},
 note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
 year = 2014
}

@article{karras2017progressive,
  title={Progressive growing of gans for improved quality, stability, and variation},
  author={Karras, Tero and Aila, Timo and Laine, Samuli and Lehtinen, Jaakko},
  journal={arXiv preprint arXiv:1710.10196},
  year={2017}
}

@article{parmar2023zero,
  title={Zero-shot image-to-image translation},
  author={Parmar, Gaurav and Singh, Krishna Kumar and Zhang, Richard and Li, Yijun and Lu, Jingwan and Zhu, Jun-Yan},
  journal={arXiv preprint arXiv:2302.03027},
  year={2023}
}

@inproceedings{gong2019autogan,
  title={Autogan: Neural architecture search for generative adversarial networks},
  author={Gong, Xinyu and Chang, Shiyu and Jiang, Yifan and Wang, Zhangyang},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={3224--3234},
  year={2019}
}

@misc{Authors14b,
 author = {Full Author Name},
 title = {Frobnication Tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {Alvin Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12, 
number = 1, 
pages = {234--778}, 
year = 2002
}

@article{Alpher03,
author = {Alvin Alpher and Ferris P.~N. Fotheringham-Smythe},
title = {Frobnication Revisited},
journal = {Journal of Foo},
volume = 13, 
number = 1, 
pages = {234--778}, 
year = 2003
}

@article{Alpher04,
author = {Alvin Alpher and Ferris P.~N. Fotheringham-Smythe and Gavin Gamow},
title = {Can a Machine Frobnicate?},
journal = {Journal of Foo},
volume = 14, 
number = 1, 
pages = {234--778}, 
year = 2004
}

@article{williams2023structured,
  title={Structured Generative Models for Scene Understanding},
  author={Williams, Christopher KI},
  journal={arXiv preprint arXiv:2302.03531},
  year={2023}
}

@inproceedings{jain2023oneformer,
  title={Oneformer: One transformer to rule universal image segmentation},
  author={Jain, Jitesh and Li, Jiachen and Chiu, Mang Tik and Hassani, Ali and Orlov, Nikita and Shi, Humphrey},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2989--2998},
  year={2023}
}

@article{jain2021semask,
  title={SeMask: Semantically Masking Transformer Backbones for Effective Semantic Segmentation},
  author={Jitesh Jain and Anukriti Singh and Nikita Orlov and Zilong Huang and Jiachen Li and Steven Walton and Humphrey Shi},
  journal={arXiv},
  year={2021}
}

@inproceedings{zeiler2014visualizing,
  title={Visualizing and understanding convolutional networks},
  author={Zeiler, Matthew D and Fergus, Rob},
  booktitle={Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part I 13},
  pages={818--833},
  year={2014},
  organization={Springer}
}

@article{yosinski2015understanding,
  title={Understanding neural networks through deep visualization},
  author={Yosinski, Jason and Clune, Jeff and Nguyen, Anh and Fuchs, Thomas and Lipson, Hod},
  journal={arXiv preprint arXiv:1506.06579},
  year={2015}
}

@article{gatys2015neural,
  title={A neural algorithm of artistic style},
  author={Gatys, Leon A and Ecker, Alexander S and Bethge, Matthias},
  journal={arXiv preprint arXiv:1508.06576},
  year={2015}
}

@InProceedings{Brown2022E2EVE,
  author       = "Andrew Brown and Cheng-Yang Fu and Omkar Parkhi and Tamara L. Berg and Andrea Vedaldi",
  title        = "End-to-End Visual Editing with a Generatively Pre-Trained Artist",
  booktitle    = "European Conference on Computer Vision (ECCV)",
  year         = "2022",
}

@inproceedings{huang2017arbitrary,
  title={Arbitrary style transfer in real-time with adaptive instance normalization},
  author={Huang, Xun and Belongie, Serge},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1501--1510},
  year={2017}
}

@inproceedings{kalischek2021light,
  title={In the light of feature distributions: moment matching for neural style transfer},
  author={Kalischek, Nikolai and Wegner, Jan D and Schindler, Konrad},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9382--9391},
  year={2021}
}

@article{huk2022shape,
  title={Shape-Guided Diffusion with Inside-Outside Attention},
  author={Huk Park, Dong and Luo, Grace and Toste, Clayton and Azadi, Samaneh and Liu, Xihui and Karalashvili, Maka and Rohrbach, Anna and Darrell, Trevor},
  journal={arXiv e-prints},
  pages={arXiv--2212},
  year={2022}
}

@article{qi2022open,
  title={Open World Entity Segmentation},
  author={Qi, Lu and Kuen, Jason and Wang, Yi and Gu, Jiuxiang and Zhao, Hengshuang and Torr, Philip and Lin, Zhe and Jia, Jiaya},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}

@misc{xu22versatile,
  url = {https://arxiv.org/abs/2211.08332},
  author = {Xu, Xingqian and Wang, Zhangyang and Zhang, Eric and Wang, Kai and Shi, Humphrey},
  title = {Versatile Diffusion: Text, Images and Variations All in One Diffusion Model},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{cheng2022masked,
  title={Masked-attention mask transformer for universal image segmentation},
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G and Kirillov, Alexander and Girdhar, Rohit},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={1290--1299},
  year={2022}
}

@inproceedings{zhou2017scene,
  title={Scene parsing through ade20k dataset},
  author={Zhou, Bolei and Zhao, Hang and Puig, Xavier and Fidler, Sanja and Barriuso, Adela and Torralba, Antonio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={633--641},
  year={2017}
}




@inproceedings{deng2019arcface,
  title={Arcface: Additive angular margin loss for deep face recognition},
  author={Deng, Jiankang and Guo, Jia and Xue, Niannan and Zafeiriou, Stefanos},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4690--4699},
  year={2019}
}

@inproceedings{CelebAMask-HQ,
  title={MaskGAN: Towards Diverse and Interactive Facial Image Manipulation},
  author={Lee, Cheng-Han and Liu, Ziwei and Wu, Lingyun and Luo, Ping},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2020}
}

@inproceedings{caesar2018coco,
  title={Coco-stuff: Thing and stuff classes in context},
  author={Caesar, Holger and Uijlings, Jasper and Ferrari, Vittorio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1209--1218},
  year={2018}
}

@misc{schuhmann2021laion400m,
      title={LAION-400M: Open Dataset of CLIP-Filtered 400 Million Image-Text Pairs}, 
      author={Christoph Schuhmann and Richard Vencu and Romain Beaumont and Robert Kaczmarczyk and Clayton Mullis and Aarush Katta and Theo Coombes and Jenia Jitsev and Aran Komatsuzaki},
      year={2021},
      eprint={2111.02114},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}


@misc{epstein_blobgan_2022,
	title = {{BlobGAN}: {Spatially} {Disentangled} {Scene} {Representations}},
	shorttitle = {{BlobGAN}},
	url = {http://arxiv.org/abs/2205.02837},
	abstract = {We propose an unsupervised, mid-level representation for a generative model of scenes. The representation is mid-level in that it is neither per-pixel nor per-image; rather, scenes are modeled as a collection of spatial, depth-ordered "blobs" of features. Blobs are differentiably placed onto a feature grid that is decoded into an image by a generative adversarial network. Due to the spatial uniformity of blobs and the locality inherent to convolution, our network learns to associate different blobs with different entities in a scene and to arrange these blobs to capture scene layout. We demonstrate this emergent behavior by showing that, despite training without any supervision, our method enables applications such as easy manipulation of objects within a scene (e.g., moving, removing, and restyling furniture), creation of feasible scenes given constraints (e.g., plausible rooms with drawers at a particular location), and parsing of real-world images into constituent parts. On a challenging multi-category dataset of indoor scenes, BlobGAN outperforms StyleGAN2 in image quality as measured by FID. See our project page for video results and interactive demo: https://www.dave.ml/blobgan},
	urldate = {2022-11-01},
	publisher = {arXiv},
	author = {Epstein, Dave and Park, Taesung and Zhang, Richard and Shechtman, Eli and Efros, Alexei A.},
	month = jul,
	year = {2022},
	note = {arXiv:2205.02837 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: ECCV 2022. Project webpage available at https://www.dave.ml/blobgan},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/5L879WLR/Epstein et al. - 2022 - BlobGAN Spatially Disentangled Scene Representati.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/G9M5JJV8/2205.html:text/html},
}

@misc{zou_ilsgan_2022,
	title = {{ILSGAN}: {Independent} {Layer} {Synthesis} for {Unsupervised} {Foreground}-{Background} {Segmentation}},
	shorttitle = {{ILSGAN}},
	url = {http://arxiv.org/abs/2211.13974},
	abstract = {Unsupervised foreground-background segmentation aims at extracting salient objects from cluttered backgrounds, where Generative Adversarial Network (GAN) approaches, especially layered GANs, show great promise. However, without human annotations, they are typically prone to produce foreground and background layers with non-negligible semantic and visual confusion, dubbed ``information leakage", resulting in notable degeneration of the generated segmentation mask. To alleviate this issue, we propose a simple-yet-effective explicit layer independence modeling approach, termed Independent Layer Synthesis GAN (ILSGAN), pursuing independent foreground-background layer generation by encouraging their discrepancy. Specifically, it targets minimizing the mutual information between visible and invisible regions of the foreground and background to spur interlayer independence. Through in-depth theoretical and experimental analyses, we justify that explicit layer independence modeling is critical to suppressing information leakage and contributes to impressive segmentation performance gains. Also, our ILSGAN achieves strong state-of-the-art generation quality and segmentation performance on complex real-world data. The code is available in the supplementary material.},
	urldate = {2022-11-28},
	publisher = {arXiv},
	author = {Zou, Qiran and Yang, Yu and Cheung, Wing Yin and Liu, Chang and Ji, Xiangyang},
	month = nov,
	year = {2022},
	note = {arXiv:2211.13974 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	annote = {Comment: Accepted by AAAI 2023},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/787DREVV/Zou et al. - 2022 - ILSGAN Independent Layer Synthesis for Unsupervis.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/7IZFFPFF/2211.html:text/html},
}

@misc{ling_editgan_2021,
	title = {{EditGAN}: {High}-{Precision} {Semantic} {Image} {Editing}},
	shorttitle = {{EditGAN}},
	url = {http://arxiv.org/abs/2111.03186},
	abstract = {Generative adversarial networks (GANs) have recently found applications in image editing. However, most GAN based image editing methods often require large scale datasets with semantic segmentation annotations for training, only provide high level control, or merely interpolate between different images. Here, we propose EditGAN, a novel method for high quality, high precision semantic image editing, allowing users to edit images by modifying their highly detailed part segmentation masks, e.g., drawing a new mask for the headlight of a car. EditGAN builds on a GAN framework that jointly models images and their semantic segmentations, requiring only a handful of labeled examples, making it a scalable tool for editing. Specifically, we embed an image into the GAN latent space and perform conditional latent code optimization according to the segmentation edit, which effectively also modifies the image. To amortize optimization, we find editing vectors in latent space that realize the edits. The framework allows us to learn an arbitrary number of editing vectors, which can then be directly applied on other images at interactive rates. We experimentally show that EditGAN can manipulate images with an unprecedented level of detail and freedom, while preserving full image quality.We can also easily combine multiple edits and perform plausible edits beyond EditGAN training data. We demonstrate EditGAN on a wide variety of image types and quantitatively outperform several previous editing methods on standard editing benchmark tasks.},
	urldate = {2023-01-26},
	publisher = {arXiv},
	author = {Ling, Huan and Kreis, Karsten and Li, Daiqing and Kim, Seung Wook and Torralba, Antonio and Fidler, Sanja},
	month = nov,
	year = {2021},
	note = {arXiv:2111.03186 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/SJIY6Z6L/Ling et al. - 2021 - EditGAN High-Precision Semantic Image Editing.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/GRD2YVCS/2111.html:text/html},
}

@article{sushko_one-shot_nodate,
	title = {One-{Shot} {Synthesis} of {Images} and {Segmentation} {Masks}},
	abstract = {Joint synthesis of images and segmentation masks with generative adversarial networks (GANs) is promising to reduce the effort needed for collecting image data with pixel-wise annotations. However, to learn high-ﬁdelity image-mask synthesis, existing GAN approaches ﬁrst need a pre-training phase requiring large amounts of image data, which limits their utilization in restricted image domains. In this work, we take a step to reduce this limitation, introducing the task of one-shot image-mask synthesis. We aim to generate diverse images and their segmentation masks given only a single labelled example, and assuming, contrary to previous models, no access to any pre-training data. To this end, inspired by the recent architectural developments of single-image GANs, we introduce our OSMIS model which enables the synthesis of segmentation masks that are precisely aligned to the generated images in the one-shot regime. Besides achieving the high ﬁdelity of generated masks, OSMIS outperforms state-of-the-art single-image GAN models in image synthesis quality and diversity. In addition, despite not using any additional data, OSMIS demonstrates an impressive ability to serve as a source of useful data augmentation for one-shot segmentation applications, providing performance gains that are complementary to standard data augmentation techniques. Code is available at https://github.com/ boschresearch/one-shot-synthesis.},
	language = {en},
	author = {Sushko, Vadim and Zhang, Dan and Gall, Jurgen and Khoreva, Anna},
	file = {Sushko et al. - One-Shot Synthesis of Images and Segmentation Mask.pdf:/Users/viditgeol/Zotero/storage/NZCHWWNV/Sushko et al. - One-Shot Synthesis of Images and Segmentation Mask.pdf:application/pdf},
}

@misc{zhu_linkgan_2023,
	title = {{LinkGAN}: {Linking} {GAN} {Latents} to {Pixels} for {Controllable} {Image} {Synthesis}},
	shorttitle = {{LinkGAN}},
	url = {http://arxiv.org/abs/2301.04604},
	abstract = {This work presents an easy-to-use regularizer for GAN training, which helps explicitly link some axes of the latent space to an image region or a semantic category (e.g., sky) in the synthesis. Establishing such a connection facilitates a more convenient local control of GAN generation, where users can alter image content only within a spatial area simply by partially resampling the latent codes. Experimental results confirm four appealing properties of our regularizer, which we call LinkGAN. (1) Any image region can be linked to the latent space, even if the region is pre-selected before training and fixed for all instances. (2) Two or multiple regions can be independently linked to different latent axes, surprisingly allowing tokenized control of synthesized images. (3) Our regularizer can improve the spatial controllability of both 2D and 3D GAN models, barely sacrificing the synthesis performance. (4) The models trained with our regularizer are compatible with GAN inversion techniques and maintain editability on real images},
	urldate = {2023-01-26},
	publisher = {arXiv},
	author = {Zhu, Jiapeng and Yang, Ceyuan and Shen, Yujun and Shi, Zifan and Zhao, Deli and Chen, Qifeng},
	month = jan,
	year = {2023},
	note = {arXiv:2301.04604 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/RFW4Z5IA/Zhu et al. - 2023 - LinkGAN Linking GAN Latents to Pixels for Control.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/ZEAHBPU2/2301.html:text/html},
}

@misc{sauer_stylegan-t_2023,
	title = {{StyleGAN}-{T}: {Unlocking} the {Power} of {GANs} for {Fast} {Large}-{Scale} {Text}-to-{Image} {Synthesis}},
	shorttitle = {{StyleGAN}-{T}},
	url = {http://arxiv.org/abs/2301.09515},
	doi = {10.48550/arXiv.2301.09515},
	abstract = {Text-to-image synthesis has recently seen significant progress thanks to large pretrained language models, large-scale training data, and the introduction of scalable model families such as diffusion and autoregressive models. However, the best-performing models require iterative evaluation to generate a single sample. In contrast, generative adversarial networks (GANs) only need a single forward pass. They are thus much faster, but they currently remain far behind the state-of-the-art in large-scale text-to-image synthesis. This paper aims to identify the necessary steps to regain competitiveness. Our proposed model, StyleGAN-T, addresses the specific requirements of large-scale text-to-image synthesis, such as large capacity, stable training on diverse datasets, strong text alignment, and controllable variation vs. text alignment tradeoff. StyleGAN-T significantly improves over previous GANs and outperforms distilled diffusion models - the previous state-of-the-art in fast text-to-image synthesis - in terms of sample quality and speed.},
	urldate = {2023-01-28},
	publisher = {arXiv},
	author = {Sauer, Axel and Karras, Tero and Laine, Samuli and Geiger, Andreas and Aila, Timo},
	month = jan,
	year = {2023},
	note = {arXiv:2301.09515 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
	annote = {Comment: Project page: https://sites.google.com/view/stylegan-t/},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/8QVK2EFQ/Sauer et al. - 2023 - StyleGAN-T Unlocking the Power of GANs for Fast L.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/DSQKCDEX/2301.html:text/html},
}

@misc{collins_editing_2020,
	title = {Editing in {Style}: {Uncovering} the {Local} {Semantics} of {GANs}},
	shorttitle = {Editing in {Style}},
	url = {http://arxiv.org/abs/2004.14367},
	doi = {10.48550/arXiv.2004.14367},
	abstract = {While the quality of GAN image synthesis has improved tremendously in recent years, our ability to control and condition the output is still limited. Focusing on StyleGAN, we introduce a simple and effective method for making local, semantically-aware edits to a target output image. This is accomplished by borrowing elements from a source image, also a GAN output, via a novel manipulation of style vectors. Our method requires neither supervision from an external model, nor involves complex spatial morphing operations. Instead, it relies on the emergent disentanglement of semantic objects that is learned by StyleGAN during its training. Semantic editing is demonstrated on GANs producing human faces, indoor scenes, cats, and cars. We measure the locality and photorealism of the edits produced by our method, and find that it accomplishes both.},
	urldate = {2023-01-28},
	publisher = {arXiv},
	author = {Collins, Edo and Bala, Raja and Price, Bob and Süsstrunk, Sabine},
	month = may,
	year = {2020},
	note = {arXiv:2004.14367 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
	annote = {Comment: IEEE Conference on Computer Vision and Patten Recognition (CVPR), 2020. Code: https://github.com/IVRL/GANLocalEditing},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/VM2T45P6/Collins et al. - 2020 - Editing in Style Uncovering the Local Semantics o.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/ZJ9SN6YF/2004.html:text/html},
}


@inproceedings{collins2020editing,
  title={Editing in Style: Uncovering the Local Semantics of GANs},
  author={Collins, Edo and Bala, Raja and Price, Bob and Susstrunk, Sabine},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5771--5780},
  year={2020}
}
@inproceedings{shen2020interpreting,
  title={Interpreting the latent space of gans for semantic face editing},
  author={Shen, Yujun and Gu, Jinjin and Tang, Xiaoou and Zhou, Bolei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={9243--9252},
  year={2020}
}

@inproceedings{karras2020analyzing,
  title={Analyzing and improving the image quality of stylegan},
  author={Karras, Tero and Laine, Samuli and Aittala, Miika and Hellsten, Janne and Lehtinen, Jaakko and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={8110--8119},
  year={2020}
}

@inproceedings{collins2018deep,
  title={Deep feature factorization for concept discovery},
  author={Collins, Edo and Achanta, Radhakrishna and Susstrunk, Sabine},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={336--352},
  year={2018}
}
@article{shen2020closed,
  title={Closed-Form Factorization of Latent Semantics in GANs},
  author={Shen, Yujun and Zhou, Bolei},
  journal={arXiv preprint arXiv:2007.06600},
  year={2020}
}
@inproceedings{zhudomain,
  title={In-Domain GAN Inversion for Real Image Editing Supplementary Material},
  author={Zhu, Jiapeng and Shen, Yujun and Zhao, Deli and Zhou, Bolei},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2020}
}
@inproceedings{bau2020rewriting,
  title={Rewriting a Deep Generative Model},
  author={Bau, David and Liu, Steven and Wang, Tongzhou and Zhu, Jun-Yan and Torralba, Antonio},
  booktitle={Proceedings of European Conference on Computer Vision (ECCV)},
  year={2020}
}
@inproceedings{jahanian2019steerability,
  title={On the''steerability" of generative adversarial networks},
  author={Jahanian, Ali and Chai, Lucy and Isola, Phillip},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2020}
}
@article{bau2020semantic,
  title={Semantic photo manipulation with a generative image prior},
  author={Bau, David and Strobelt, Hendrik and Peebles, William and Zhou, Bolei and Zhu, Jun-Yan and Torralba, Antonio and others},
  journal={ACM Transactions on Graphics (ToG)},
  year={2019}
}

@inproceedings{bau2018gan,
  title={Gan dissection: Visualizing and understanding generative adversarial networks},
  author={Bau, David and Zhu, Jun-Yan and Strobelt, Hendrik and Zhou, Bolei and Tenenbaum, Joshua B and Freeman, William T and Torralba, Antonio},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2019}
}
@inproceedings{huh2020transforming,
  title={Transforming and Projecting Images into Class-conditional Generative Networks},
  author={Huh, Minyoung and Zhang, Richard and Zhu, Jun-Yan and Paris, Sylvain and Hertzmann, Aaron},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  year={2020}
}
@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in Neural Information Processing Systems (NeurIPS)},
  pages={2672--2680},
  year={2014}
}
@inproceedings{brock2018large,
  title={Large scale gan training for high fidelity natural image synthesis},
  author={Brock, Andrew and Donahue, Jeff and Simonyan, Karen},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2019}
}
@article{suzuki2018spatially,
  title={Spatially controllable image synthesis with internal representation collaging},
  author={Suzuki, Ryohei and Koyama, Masanori and Miyato, Takeru and Yonetsuji, Taizan and Zhu, Huachun},
  journal={arXiv preprint arXiv:1811.10153},
  year={2018}
}
@inproceedings{bau2019seeing,
  title={Seeing what a gan cannot generate},
  author={Bau, David and Zhu, Jun-Yan and Wulff, Jonas and Peebles, William and Strobelt, Hendrik and Zhou, Bolei and Torralba, Antonio},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  pages={4502--4511},
  year={2019}
}
@article{hin2019interactive,
  title={Interactive Subspace Exploration on Generative Image Modelling},
  author={Hin, Toby Chong Long and Shen, I and Sato, Issei and Igarashi, Takeo and others},
  journal={arXiv preprint arXiv:1906.09840},
  year={2019}
}
@inproceedings{bau2017network,
  title={Network dissection: Quantifying interpretability of deep visual representations},
  author={Bau, David and Zhou, Bolei and Khosla, Aditya and Oliva, Aude and Torralba, Antonio},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={6541--6549},
  year={2017}
}
@article{bau2020understanding,
  title={Understanding the role of individual units in a deep neural network},
  author={Bau, David and Zhu, Jun-Yan and Strobelt, Hendrik and Lapedriza, Agata and Zhou, Bolei and Torralba, Antonio},
  journal={Proceedings of the National Academy of Sciences (PNAS)},
  year={2020},
  publisher={National Acad Sciences}
}

@inproceedings{gu2020image,
  title={Image processing using multi-code gan prior},
  author={Gu, Jinjin and Shen, Yujun and Zhou, Bolei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={3012--3021},
  year={2020}
}
@inproceedings{zhou2016learning,
  title={Learning deep features for discriminative localization},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={2921--2929},
  year={2016}
}
@article{yu2015lsun,
  title={Lsun: Construction of a large-scale image dataset using deep learning with humans in the loop},
  author={Yu, Fisher and Seff, Ari and Zhang, Yinda and Song, Shuran and Funkhouser, Thomas and Xiao, Jianxiong},
  journal={arXiv preprint arXiv:1506.03365},
  year={2015}
}

@inproceedings{huang2017arbitrary,
  title={Arbitrary style transfer in real-time with adaptive instance normalization},
  author={Huang, Xun and Belongie, Serge},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  pages={1501--1510},
  year={2017}
}

@inproceedings{donahue2014decaf,
  title={Decaf: A deep convolutional activation feature for generic visual recognition},
  author={Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
  booktitle={International Conference on Machine Learning (ICML)},
  pages={647--655},
  year={2014}
}
@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}
@article{krizhevsky2017imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Communications of the ACM},
  volume={60},
  number={6},
  pages={84--90},
  year={2017},
  publisher={ACM New York, NY, USA}
}
@inproceedings{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2015}
}
@inproceedings{lee2020maskgan,
  title={Maskgan: Towards diverse and interactive facial image manipulation},
  author={Lee, Cheng-Han and Liu, Ziwei and Wu, Lingyun and Luo, Ping},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5549--5558},
  year={2020}
}
@inproceedings{wang2020attentive,
  title={Attentive Normalization for Conditional Image Generation},
  author={Wang, Yi and Chen, Ying-Cong and Zhang, Xiangyu and Sun, Jian and Jia, Jiaya},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5094--5103},
  year={2020}
}
@inproceedings{besserve2018counterfactuals,
  title={Counterfactuals uncover the modular structure of deep generative models},
  author={Besserve, Michel and Mehrjou, Arash and Sun, R{\'e}my and Sch{\"o}lkopf, Bernhard},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2020}
}
@inproceedings{plumerault2020controlling,
  title={Controlling generative models with continuous factors of variations},
  author={Plumerault, Antoine and Borgne, Herv{\'e} Le and Hudelot, C{\'e}line},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2020}
}
@article{olah2018the,
  author = {Olah, Chris and Satyanarayan, Arvind and Johnson, Ian and Carter, Shan and Schubert, Ludwig and Ye, Katherine and Mordvintsev, Alexander},
  title = {The Building Blocks of Interpretability},
  journal = {Distill},
  year = {2018},
  note = {https://distill.pub/2018/building-blocks},
  doi = {10.23915/distill.00010}
}
@article{zhou2018revisiting,
  title={Revisiting the importance of individual units in cnns via ablation},
  author={Zhou, Bolei and Sun, Yiyou and Bau, David and Torralba, Antonio},
  journal={arXiv preprint arXiv:1806.02891},
  year={2018}
}
@inproceedings{zhang2018interpretable,
  title={Interpretable convolutional neural networks},
  author={Zhang, Quanshi and Nian Wu, Ying and Zhu, Song-Chun},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={8827--8836},
  year={2018}
}
@inproceedings{huang2018multimodal,
  title={Multimodal unsupervised image-to-image translation},
  author={Huang, Xun and Liu, Ming-Yu and Belongie, Serge and Kautz, Jan},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={172--189},
  year={2018}
}
@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1125--1134},
  year={2017}
}
@inproceedings{heusel2017gans,
  title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
  author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
  booktitle={Advances in Neural Information Processing Systems (NeurIPS)},
  pages={6626--6637},
  year={2017}
}
@inproceedings{miyato2018spectral,
  title={Spectral normalization for generative adversarial networks},
  author={Miyato, Takeru and Kataoka, Toshiki and Koyama, Masanori and Yoshida, Yuichi},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2018}
}

@inproceedings{sangkloy2017scribbler,
  title={Scribbler: Controlling deep image synthesis with sketch and color},
  author={Sangkloy, Patsorn and Lu, Jingwan and Fang, Chen and Yu, Fisher and Hays, James},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={5400--5409},
  year={2017}
}
@inproceedings{wang2018video,
  title={Video-to-video synthesis},
  author={Wang, Ting-Chun and Liu, Ming-Yu and Zhu, Jun-Yan and Liu, Guilin and Tao, Andrew and Kautz, Jan and Catanzaro, Bryan},
  booktitle={Advances in Neural Information Processing Systems (NeurIPS)},
  year={2018}
}
@inproceedings{agustsson2019generative,
  title={Generative adversarial networks for extreme learned image compression},
  author={Agustsson, Eirikur and Tschannen, Michael and Mentzer, Fabian and Timofte, Radu and Gool, Luc Van},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  pages={221--231},
  year={2019}
}

@inproceedings{ledig2017photo,
  title={Photo-realistic single image super-resolution using a generative adversarial network},
  author={Ledig, Christian and Theis, Lucas and Husz{\'a}r, Ferenc and Caballero, Jose and Cunningham, Andrew and Acosta, Alejandro and Aitken, Andrew and Tejani, Alykhan and Totz, Johannes and Wang, Zehan and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={4681--4690},
  year={2017}
}
@incollection{mundra2019video,
  title={Video DeCaptioning Using U-Net with Stacked Dilated Convolutional Layers},
  author={Mundra, Shivansh and Jain, Arnav Kumar and Sinha, Sayan},
  booktitle={Inpainting and Denoising Challenges},
  pages={77--86},
  year={2019},
  publisher={Springer}
}
@inproceedings{liao2018face,
  title={Face completion with semantic knowledge and collaborative adversarial learning},
  author={Liao, Haofu and Funka-Lea, Gareth and Zheng, Yefeng and Luo, Jiebo and Zhou, S Kevin},
  booktitle={Asian Conference on Computer Vision (ACCV)},
  pages={382--397},
  year={2018},
  organization={Springer}
}
@inproceedings{dolhansky2018eye,
  title={Eye in-painting with exemplar generative adversarial networks},
  author={Dolhansky, Brian and Canton Ferrer, Cristian},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={7902--7911},
  year={2018}
}

@inproceedings{2020ganspace,
  title     = {GANSpace: Discovering Interpretable GAN Controls},
  author    = {Erik Härkönen and Aaron Hertzmann and Jaakko Lehtinen and Sylvain Paris},
  booktitle = {Proc. NeurIPS},
  year      = {2020}
}
@misc{esser2020taming,
      title={Taming Transformers for High-Resolution Image Synthesis}, 
      author={Patrick Esser and Robin Rombach and Björn Ommer},
      year={2020},
      eprint={2012.09841},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@article{jiang2021transgan,
  title={Transgan: Two transformers can make one strong gan},
  author={Jiang, Yifan and Chang, Shiyu and Wang, Zhangyang},
  journal={arXiv preprint arXiv:2102.07074},
  year={2021}
}

@article{yang2021semantic,
  title={Semantic hierarchy emerges in deep generative representations for scene synthesis},
  author={Yang, Ceyuan and Shen, Yujun and Zhou, Bolei},
  journal={International Journal of Computer Vision},
  pages={1--16},
  year={2021},
  publisher={Springer}
}

@article{li2022diffusion,
  title={Diffusion-lm improves controllable text generation},
  author={Li, Xiang Lisa and Thickstun, John and Gulrajani, Ishaan and Liang, Percy and Hashimoto, Tatsunori B},
  journal={arXiv preprint arXiv:2205.14217},
  year={2022}
}

@inproceedings{patashnik2021styleclip,
  title={Styleclip: Text-driven manipulation of stylegan imagery},
  author={Patashnik, Or and Wu, Zongze and Shechtman, Eli and Cohen-Or, Daniel and Lischinski, Dani},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2085--2094},
  year={2021}
}

@inproceedings{park2022styleformer,
  title={Styleformer: Transformer based generative adversarial networks with style vector},
  author={Park, Jeeseung and Kim, Younggeun},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8983--8992},
  year={2022}
}

@article{radford2015unsupervised,
  title={Unsupervised representation learning with deep convolutional generative adversarial networks},
  author={Radford, Alec and Metz, Luke and Chintala, Soumith},
  journal={arXiv preprint arXiv:1511.06434},
  year={2015}
}

@article{schuhmann2022laion,
  title={Laion-5b: An open large-scale dataset for training next generation image-text models},
  author={Schuhmann, Christoph and Beaumont, Romain and Vencu, Richard and Gordon, Cade and Wightman, Ross and Cherti, Mehdi and Coombes, Theo and Katta, Aarush and Mullis, Clayton and Wortsman, Mitchell and others},
  journal={arXiv preprint arXiv:2210.08402},
  year={2022}
}

@inproceedings{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={International conference on machine learning},
  pages={8748--8763},
  year={2021},
  organization={PMLR}
}

@inproceedings{abdal2020image2stylegan++,
  title={Image2stylegan++: How to edit the embedded images?},
  author={Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={8296--8305},
  year={2020}
}

@inproceedings{zhu2016generative,
  title={Generative visual manipulation on the natural image manifold},
  author={Zhu, Jun-Yan and Kr{\"a}henb{\"u}hl, Philipp and Shechtman, Eli and Efros, Alexei A},
  booktitle={Computer Vision--ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part V 14},
  pages={597--613},
  year={2016},
  organization={Springer}
}

@article{perarnau2016invertible,
  title={Invertible conditional gans for image editing},
  author={Perarnau, Guim and Van De Weijer, Joost and Raducanu, Bogdan and {\'A}lvarez, Jose M},
  journal={arXiv preprint arXiv:1611.06355},
  year={2016}
}

@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}



@inproceedings{bora2017compressed,
  title={Compressed sensing using generative models},
  author={Bora, Ashish and Jalal, Ajil and Price, Eric and Dimakis, Alexandros G},
  booktitle={International Conference on Machine Learning},
  pages={537--546},
  year={2017},
  organization={PMLR}
}

@article{mokady2022null,
  title={Null-text Inversion for Editing Real Images using Guided Diffusion Models},
  author={Mokady, Ron and Hertz, Amir and Aberman, Kfir and Pritch, Yael and Cohen-Or, Daniel},
  journal={arXiv preprint arXiv:2211.09794},
  year={2022}
}

@inproceedings{wu2021stylespace,
  title={Stylespace analysis: Disentangled controls for stylegan image generation},
  author={Wu, Zongze and Lischinski, Dani and Shechtman, Eli},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12863--12872},
  year={2021}
}

@inproceedings{abdal2019image2stylegan,
  title={Image2stylegan: How to embed images into the stylegan latent space?},
  author={Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4432--4441},
  year={2019}
}

@inproceedings{karras2019style,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4401--4410},
  year={2019}
}

@article{couairon2022diffedit,
  title={Diffedit: Diffusion-based semantic image editing with mask guidance},
  author={Couairon, Guillaume and Verbeek, Jakob and Schwenk, Holger and Cord, Matthieu},
  journal={arXiv preprint arXiv:2210.11427},
  year={2022}
}

@article{zhang2023adding,
  title={Adding Conditional Control to Text-to-Image Diffusion Models},
  author={Zhang, Lvmin and Agrawala, Maneesh},
  journal={arXiv preprint arXiv:2302.05543},
  year={2023}
}

@article{wang2022semantic,
  title={Semantic image synthesis via diffusion models},
  author={Wang, Weilun and Bao, Jianmin and Zhou, Wengang and Chen, Dongdong and Chen, Dong and Yuan, Lu and Li, Houqiang},
  journal={arXiv preprint arXiv:2207.00050},
  year={2022}
}

@article{yang2022diffusion,
  title={Diffusion-Based Scene Graph to Image Generation with Masked Contrastive Pre-Training},
  author={Yang, Ling and Huang, Zhilin and Song, Yang and Hong, Shenda and Li, Guohao and Zhang, Wentao and Cui, Bin and Ghanem, Bernard and Yang, Ming-Hsuan},
  journal={arXiv preprint arXiv:2211.11138},
  year={2022}
}

@article{hertz2022prompt,
  title={Prompt-to-prompt image editing with cross attention control},
  author={Hertz, Amir and Mokady, Ron and Tenenbaum, Jay and Aberman, Kfir and Pritch, Yael and Cohen-Or, Daniel},
  journal={arXiv preprint arXiv:2208.01626},
  year={2022}
}



@article{huang2023composer,
  title={Composer: Creative and Controllable Image Synthesis with Composable Conditions},
  author={Huang, Lianghua and Chen, Di and Liu, Yu and Shen, Yujun and Zhao, Deli and Zhou, Jingren},
  journal={arXiv preprint arXiv:2302.09778},
  year={2023}
}

@inproceedings{cheng2023adaptively,
  title={Adaptively-Realistic Image Generation from Stroke and Sketch with Diffusion Model},
  author={Cheng, Shin-I and Chen, Yu-Jie and Chiu, Wei-Chen and Tseng, Hung-Yu and Lee, Hsin-Ying},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={4054--4062},
  year={2023}
}

@article{zeng2022scenecomposer,
  title={SceneComposer: Any-Level Semantic Image Synthesis},
  author={Zeng, Yu and Lin, Zhe and Zhang, Jianming and Liu, Qing and Collomosse, John and Kuen, Jason and Patel, Vishal M},
  journal={arXiv preprint arXiv:2211.11742},
  year={2022}
}

@article{cheng2023play,
  title={PLay: Parametrically Conditioned Layout Generation using Latent Diffusion},
  author={Cheng, Chin-Yi and Huang, Forrest and Li, Gang and Li, Yang},
  journal={arXiv preprint arXiv:2301.11529},
  year={2023}
}

@article{kwon2022diffusion,
  title={Diffusion-based image translation using disentangled style and content representation},
  author={Kwon, Gihyun and Ye, Jong Chul},
  journal={arXiv preprint arXiv:2209.15264},
  year={2022}
}

@inproceedings{zhu2020sean,
  title={Sean: Image synthesis with semantic region-adaptive normalization},
  author={Zhu, Peihao and Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5104--5113},
  year={2020}
}

@inproceedings{park2019semantic,
  title={Semantic image synthesis with spatially-adaptive normalization},
  author={Park, Taesung and Liu, Ming-Yu and Wang, Ting-Chun and Zhu, Jun-Yan},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2337--2346},
  year={2019}
}



@inproceedings{xian2018texturegan,
  title={Texturegan: Controlling deep image synthesis with texture patches},
  author={Xian, Wenqi and Sangkloy, Patsorn and Agrawal, Varun and Raj, Amit and Lu, Jingwan and Fang, Chen and Yu, Fisher and Hays, James},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8456--8465},
  year={2018}
}

@article{rouhsedaghat2022magic,
  title={MAGIC: Mask-Guided Image Synthesis by Inverting a Quasi-Robust Classifier},
  author={Rouhsedaghat, Mozhdeh and Monajatipoor, Masoud and Chang, Kai-Wei and Kuo, C-C Jay and Masi, Iacopo},
  journal={arXiv preprint arXiv:2209.11549},
  year={2022}
}


@inproceedings{epstein2022blobgan,
  title={Blobgan: Spatially disentangled scene representations},
  author={Epstein, Dave and Park, Taesung and Zhang, Richard and Shechtman, Eli and Efros, Alexei A},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part XV},
  pages={616--635},
  year={2022},
  organization={Springer}
}


@article{nichol2021glide,
  title={Glide: Towards photorealistic image generation and editing with text-guided diffusion models},
  author={Nichol, Alex and Dhariwal, Prafulla and Ramesh, Aditya and Shyam, Pranav and Mishkin, Pamela and McGrew, Bob and Sutskever, Ilya and Chen, Mark},
  journal={arXiv preprint arXiv:2112.10741},
  year={2021}
}

@article{dhariwal2021diffusion,
  title={Diffusion models beat gans on image synthesis},
  author={Dhariwal, Prafulla and Nichol, Alexander},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={8780--8794},
  year={2021}
}

@article{ho2022classifier,
  title={Classifier-free diffusion guidance},
  author={Ho, Jonathan and Salimans, Tim},
  journal={arXiv preprint arXiv:2207.12598},
  year={2022}
}


@inproceedings{rombach2022high,
  title={High-resolution image synthesis with latent diffusion models},
  author={Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Bj{\"o}rn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10684--10695},
  year={2022}
}

@article{singer2023text,
  title={Text-To-4D Dynamic Scene Generation},
  author={Singer, Uriel and Sheynin, Shelly and Polyak, Adam and Ashual, Oron and Makarov, Iurii and Kokkinos, Filippos and Goyal, Naman and Vedaldi, Andrea and Parikh, Devi and Johnson, Justin and others},
  journal={arXiv preprint arXiv:2301.11280},
  year={2023}
}

@article{chen2022diffusiondet,
  title={Diffusiondet: Diffusion model for object detection},
  author={Chen, Shoufa and Sun, Peize and Song, Yibing and Luo, Ping},
  journal={arXiv preprint arXiv:2211.09788},
  year={2022}
}

@article{mittal2021symbolic,
  title={Symbolic music generation with diffusion models},
  author={Mittal, Gautam and Engel, Jesse and Hawthorne, Curtis and Simon, Ian},
  journal={arXiv preprint arXiv:2103.16091},
  year={2021}
}

@article{huang2023noise2music,
  title={Noise2Music: Text-conditioned Music Generation with Diffusion Models},
  author={Huang, Qingqing and Park, Daniel S and Wang, Tao and Denk, Timo I and Ly, Andy and Chen, Nanxin and Zhang, Zhengdong and Zhang, Zhishuai and Yu, Jiahui and Frank, Christian and others},
  journal={arXiv preprint arXiv:2302.03917},
  year={2023}
}

@article{xu2022neurallift,
  title={NeuralLift-360: Lifting An In-the-wild 2D Photo to A 3D Object with 360° Views},
  author={Xu, Dejia and Jiang, Yifan and Wang, Peihao and Fan, Zhiwen and Wang, Yi and Wang, Zhangyang},
  journal={arXiv e-prints},
  pages={arXiv--2211},
  year={2022}
}

@article{poole2022dreamfusion,
  title={Dreamfusion: Text-to-3d using 2d diffusion},
  author={Poole, Ben and Jain, Ajay and Barron, Jonathan T and Mildenhall, Ben},
  journal={arXiv preprint arXiv:2209.14988},
  year={2022}
}

@article{gu2023nerfdiff,
  title={NerfDiff: Single-image View Synthesis with NeRF-guided Distillation from 3D-aware Diffusion},
  author={Gu, Jiatao and Trevithick, Alex and Lin, Kai-En and Susskind, Josh and Theobalt, Christian and Liu, Lingjie and Ramamoorthi, Ravi},
  journal={arXiv preprint arXiv:2302.10109},
  year={2023}
}

@article{ho2020denoising,
  title={Denoising diffusion probabilistic models},
  author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={6840--6851},
  year={2020}
}

@article{ho2022cascaded,
  title={Cascaded Diffusion Models for High Fidelity Image Generation},
  author={Ho, Jonathan and Saharia, Chitwan and Chan, William and Fleet, David J and Norouzi, Mohammad and Salimans, Tim},
  journal={J. Mach. Learn. Res.},
  volume={23},
  pages={47--1},
  year={2022}
}

@article{vahdat2021score,
  title={Score-based generative modeling in latent space},
  author={Vahdat, Arash and Kreis, Karsten and Kautz, Jan},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={11287--11302},
  year={2021}
}



@article{saharia2022photorealistic,
  title={Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding},
  author={Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily and Ghasemipour, Seyed Kamyar Seyed and Ayan, Burcu Karagol and Mahdavi, S Sara and Lopes, Rapha Gontijo and others},
  journal={arXiv preprint arXiv:2205.11487},
  year={2022}
}

@article{song2019generative,
  title={Generative modeling by estimating gradients of the data distribution},
  author={Song, Yang and Ermon, Stefano},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@article{ramesh2022hierarchical,
  title={Hierarchical text-conditional image generation with clip latents},
  author={Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  journal={arXiv preprint arXiv:2204.06125},
  year={2022}
}

@article{brooks2022instructpix2pix,
  title={Instructpix2pix: Learning to follow image editing instructions},
  author={Brooks, Tim and Holynski, Aleksander and Efros, Alexei A},
  journal={arXiv preprint arXiv:2211.09800},
  year={2022}
}

@misc{couairon_diffedit_2022,
	title = {{DiffEdit}: {Diffusion}-based semantic image editing with mask guidance},
	shorttitle = {{DiffEdit}},
	url = {http://arxiv.org/abs/2210.11427},
	abstract = {Image generation has recently seen tremendous advances, with diffusion models allowing to synthesize convincing images for a large variety of text prompts. In this article, we propose DiffEdit, a method to take advantage of text-conditioned diffusion models for the task of semantic image editing, where the goal is to edit an image based on a text query. Semantic image editing is an extension of image generation, with the additional constraint that the generated image should be as similar as possible to a given input image. Current editing methods based on diffusion models usually require to provide a mask, making the task much easier by treating it as a conditional inpainting task. In contrast, our main contribution is able to automatically generate a mask highlighting regions of the input image that need to be edited, by contrasting predictions of a diffusion model conditioned on different text prompts. Moreover, we rely on latent inference to preserve content in those regions of interest and show excellent synergies with mask-based diffusion. DiffEdit achieves state-of-the-art editing performance on ImageNet. In addition, we evaluate semantic image editing in more challenging settings, using images from the COCO dataset as well as text-based generated images.},
	urldate = {2022-10-26},
	publisher = {arXiv},
	author = {Couairon, Guillaume and Verbeek, Jakob and Schwenk, Holger and Cord, Matthieu},
	month = oct,
	year = {2022},
	note = {arXiv:2210.11427 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/5MQ7U5QB/Couairon et al. - 2022 - DiffEdit Diffusion-based semantic image editing w.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/67SAM64D/2210.html:text/html},
}

@misc{fan_frido_2022,
	title = {Frido: {Feature} {Pyramid} {Diffusion} for {Complex} {Scene} {Image} {Synthesis}},
	shorttitle = {Frido},
	url = {http://arxiv.org/abs/2208.13753},

	urldate = {2022-10-28},
	publisher = {arXiv},
	author = {Fan, Wan-Cyuan and Chen, Yen-Chun and Chen, DongDong and Cheng, Yu and Yuan, Lu and Wang, Yu-Chiang Frank},
	month = aug,
	year = {2022},
	note = {arXiv:2208.13753 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/N5YSFR23/Fan et al. - 2022 - Frido Feature Pyramid Diffusion for Complex Scene.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/UYYTXJEW/2208.html:text/html},
}

@misc{liew_magicmix_2022,
	title = {{MagicMix}: {Semantic} {Mixing} with {Diffusion} {Models}},
	shorttitle = {{MagicMix}},
	url = {http://arxiv.org/abs/2210.16056},
	urldate = {2022-10-31},
	publisher = {arXiv},
	author = {Liew, Jun Hao and Yan, Hanshu and Zhou, Daquan and Feng, Jiashi},
	month = oct,
	year = {2022},
	note = {arXiv:2210.16056 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/PH2ESCWQ/Liew et al. - 2022 - MagicMix Semantic Mixing with Diffusion Models.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/FP9J28BN/2210.html:text/html},
}

@misc{hertz_prompt--prompt_2022,
	title = {Prompt-to-{Prompt} {Image} {Editing} with {Cross} {Attention} {Control}},
	url = {http://arxiv.org/abs/2208.01626},
	
	urldate = {2022-10-31},
	publisher = {arXiv},
	author = {Hertz, Amir and Mokady, Ron and Tenenbaum, Jay and Aberman, Kfir and Cohen-Or, Daniel},
	month = aug,
	year = {2022},
	note = {arXiv:2208.01626 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Computer Science - Computation and Language, Computer Science - Graphics},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/7VH44CLY/Hertz et al. - 2022 - Prompt-to-Prompt Image Editing with Cross Attentio.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/38KHWJLP/2208.html:text/html},
}

@misc{rombach_high-resolution_2022,
	title = {High-{Resolution} {Image} {Synthesis} with {Latent} {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2112.10752},
	
	urldate = {2022-11-01},
	publisher = {arXiv},
	author = {Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Björn},
	month = apr,
	year = {2022},
	note = {arXiv:2112.10752 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/BGXF9KQ8/Rombach et al. - 2022 - High-Resolution Image Synthesis with Latent Diffus.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/BHEXZ3HH/2112.html:text/html},
}

@misc{balaji_ediff-i_2022,
	title = {{eDiff}-{I}: {Text}-to-{Image} {Diffusion} {Models} with an {Ensemble} of {Expert} {Denoisers}},
	shorttitle = {{eDiff}-{I}},
	url = {http://arxiv.org/abs/2211.01324},
	urldate = {2022-11-10},
	publisher = {arXiv},
	author = {Balaji, Yogesh and Nah, Seungjun and Huang, Xun and Vahdat, Arash and Song, Jiaming and Kreis, Karsten and Aittala, Miika and Aila, Timo and Laine, Samuli and Catanzaro, Bryan and Karras, Tero and Liu, Ming-Yu},
	month = nov,
	year = {2022},
	note = {arXiv:2211.01324 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/HR5ZAC5C/Balaji et al. - 2022 - eDiff-I Text-to-Image Diffusion Models with an En.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/EGUXPF7D/2211.html:text/html},
}

@misc{petsiuk_human_2022,
	title = {Human {Evaluation} of {Text}-to-{Image} {Models} on a {Multi}-{Task} {Benchmark}},
	url = {http://arxiv.org/abs/2211.12112},
	urldate = {2022-11-23},
	publisher = {arXiv},
	author = {Petsiuk, Vitali and Siemenn, Alexander E. and Surbehera, Saisamrit and Chin, Zad and Tyser, Keith and Hunter, Gregory and Raghavan, Arvind and Hicke, Yann and Plummer, Bryan A. and Kerret, Ori and Buonassisi, Tonio and Saenko, Kate and Solar-Lezama, Armando and Drori, Iddo},
	month = nov,
	year = {2022},
	note = {arXiv:2211.12112 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/6NQ4ZLB4/Petsiuk et al. - 2022 - Human Evaluation of Text-to-Image Models on a Mult.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/HSH2MFG5/2211.html:text/html},
}

@misc{liu_compositional_2022,
	title = {Compositional {Visual} {Generation} with {Composable} {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2206.01714},
	
	urldate = {2022-11-23},
	publisher = {arXiv},
	author = {Liu, Nan and Li, Shuang and Du, Yilun and Torralba, Antonio and Tenenbaum, Joshua B.},
	month = jul,
	year = {2022},
	note = {arXiv:2206.01714 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/A2MKBC9H/Liu et al. - 2022 - Compositional Visual Generation with Composable Di.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/QCVL4SKM/2206.html:text/html},
}

@article{karras_elucidating_nodate,
	title = {Elucidating the {Design} {Space} of {Diffusion}-{Based} {Generative} {Models}},
	language = {en},
	author = {Karras, Tero and Aila, Timo and Aittala, Miika and Laine, Samuli},
	pages = {48},
	file = {Karras et al. - Elucidating the Design Space of Diffusion-Based Ge.pdf:/Users/viditgeol/Zotero/storage/73A3SKLR/Karras et al. - Elucidating the Design Space of Diffusion-Based Ge.pdf:application/pdf},
}

@misc{tumanyan_plug-and-play_2022,
	title = {Plug-and-{Play} {Diffusion} {Features} for {Text}-{Driven} {Image}-to-{Image} {Translation}},
	url = {http://arxiv.org/abs/2211.12572},
	
	urldate = {2022-11-29},
	publisher = {arXiv},
	author = {Tumanyan, Narek and Geyer, Michal and Bagon, Shai and Dekel, Tali},
	month = nov,
	year = {2022},
	note = {arXiv:2211.12572 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/KUE569Z6/Tumanyan et al. - 2022 - Plug-and-Play Diffusion Features for Text-Driven I.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/5TMQSGV6/2211.html:text/html},
}

@misc{yang_reco_2022,
	title = {{ReCo}: {Region}-{Controlled} {Text}-to-{Image} {Generation}},
	shorttitle = {{ReCo}},
	url = {http://arxiv.org/abs/2211.15518},
	urldate = {2022-11-29},
	publisher = {arXiv},
	author = {Yang, Zhengyuan and Wang, Jianfeng and Gan, Zhe and Li, Linjie and Lin, Kevin and Wu, Chenfei and Duan, Nan and Liu, Zicheng and Liu, Ce and Zeng, Michael and Wang, Lijuan},
	month = nov,
	year = {2022},
	note = {arXiv:2211.15518 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/7UIZ9N9H/Yang et al. - 2022 - ReCo Region-Controlled Text-to-Image Generation.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/NQY55RGB/2211.html:text/html},
}

@misc{hu_unified_2022,
	title = {Unified {Discrete} {Diffusion} for {Simultaneous} {Vision}-{Language} {Generation}},
	url = {http://arxiv.org/abs/2211.14842},
	
	urldate = {2022-11-29},
	publisher = {arXiv},
	author = {Hu, Minghui and Zheng, Chuanxia and Zheng, Heliang and Cham, Tat-Jen and Wang, Chaoyue and Yang, Zuopeng and Tao, Dacheng and Suganthan, Ponnuthurai N.},
	month = nov,
	year = {2022},
	note = {arXiv:2211.14842 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/GVWVDGT4/Hu et al. - 2022 - Unified Discrete Diffusion for Simultaneous Vision.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/RUAK4I6N/2211.html:text/html},
}

@misc{voynov_sketch-guided_2022,
	title = {Sketch-{Guided} {Text}-to-{Image} {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2211.13752},
	
	urldate = {2022-12-03},
	publisher = {arXiv},
	author = {Voynov, Andrey and Aberman, Kfir and Cohen-Or, Daniel},
	month = nov,
	year = {2022},
	note = {arXiv:2211.13752 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Computer Science - Graphics},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/9G95CE68/Voynov et al. - 2022 - Sketch-Guided Text-to-Image Diffusion Models.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/DF692PQR/2211.html:text/html},
}

@misc{cho_dall-eval_2022,
	title = {{DALL}-{Eval}: {Probing} the {Reasoning} {Skills} and {Social} {Biases} of {Text}-to-{Image} {Generative} {Models}},
	shorttitle = {{DALL}-{Eval}},
	url = {http://arxiv.org/abs/2202.04053},
	
	urldate = {2022-12-03},
	publisher = {arXiv},
	author = {Cho, Jaemin and Zala, Abhay and Bansal, Mohit},
	month = nov,
	year = {2022},
	note = {arXiv:2202.04053 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Computation and Language},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/ISPYNEVU/Cho et al. - 2022 - DALL-Eval Probing the Reasoning Skills and Social.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/LUTWVNJV/2202.html:text/html},
}

@misc{ho_classifier-free_2022,
	title = {Classifier-{Free} {Diffusion} {Guidance}},
	url = {http://arxiv.org/abs/2207.12598},
	
	urldate = {2022-12-04},
	publisher = {arXiv},
	author = {Ho, Jonathan and Salimans, Tim},
	month = jul,
	year = {2022},
	note = {arXiv:2207.12598 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/65BVFS9B/Ho and Salimans - 2022 - Classifier-Free Diffusion Guidance.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/NBTM7KWK/2207.html:text/html},
}

@misc{zeng_scenecomposer_2022,
	title = {{SceneComposer}: {Any}-{Level} {Semantic} {Image} {Synthesis}},
	shorttitle = {{SceneComposer}},
	url = {http://arxiv.org/abs/2211.11742},
	urldate = {2022-12-04},
	publisher = {arXiv},
	author = {Zeng, Yu and Lin, Zhe and Zhang, Jianming and Liu, Qing and Collomosse, John and Kuen, Jason and Patel, Vishal M.},
	month = nov,
	year = {2022},
	note = {arXiv:2211.11742 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/Y85K55GP/Zeng et al. - 2022 - SceneComposer Any-Level Semantic Image Synthesis.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/B6KX8999/2211.html:text/html},
}

@inproceedings{chen_background_2022,
	address = {Lisboa Portugal},
	title = {Background {Layout} {Generation} and {Object} {Knowledge} {Transfer} for {Text}-to-{Image} {Generation}},
	isbn = {978-1-4503-9203-7},
	url = {https://dl.acm.org/doi/10.1145/3503161.3548154},
	doi = {10.1145/3503161.3548154},
	language = {en},
	urldate = {2022-12-05},
	booktitle = {Proceedings of the 30th {ACM} {International} {Conference} on {Multimedia}},
	publisher = {ACM},
	author = {Chen, Zhuowei and Mao, Zhendong and Fang, Shancheng and Hu, Bo},
	month = oct,
	year = {2022},
	pages = {4327--4335},
	file = {3503161.3548154.pdf:/Users/viditgeol/Downloads/3503161.3548154.pdf:application/pdf},
}

@misc{ruiz_dreambooth_2022,
	title = {{DreamBooth}: {Fine} {Tuning} {Text}-to-{Image} {Diffusion} {Models} for {Subject}-{Driven} {Generation}},
	shorttitle = {{DreamBooth}},
	url = {http://arxiv.org/abs/2208.12242},
	urldate = {2022-12-05},
	publisher = {arXiv},
	author = {Ruiz, Nataniel and Li, Yuanzhen and Jampani, Varun and Pritch, Yael and Rubinstein, Michael and Aberman, Kfir},
	month = aug,
	year = {2022},
	note = {arXiv:2208.12242 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Computer Science - Graphics},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/224NRZGT/Ruiz et al. - 2022 - DreamBooth Fine Tuning Text-to-Image Diffusion Mo.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/A82T6PN5/2208.html:text/html},
}

@misc{song_objectstitch_2022,
	title = {{ObjectStitch}: {Generative} {Object} {Compositing}},
	shorttitle = {{ObjectStitch}},
	url = {http://arxiv.org/abs/2212.00932},
	urldate = {2022-12-13},
	publisher = {arXiv},
	author = {Song, Yizhi and Zhang, Zhifei and Lin, Zhe and Cohen, Scott and Price, Brian and Zhang, Jianming and Kim, Soo Ye and Aliaga, Daniel},
	month = dec,
	year = {2022},
	note = {arXiv:2212.00932 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/JFP89N3M/Song et al. - 2022 - ObjectStitch Generative Object Compositing.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/5DMJI9T5/2212.html:text/html},
}

@misc{xie_smartbrush_2022,
	title = {{SmartBrush}: {Text} and {Shape} {Guided} {Object} {Inpainting} with {Diffusion} {Model}},
	shorttitle = {{SmartBrush}},
	url = {http://arxiv.org/abs/2212.05034},
	urldate = {2022-12-21},
	publisher = {arXiv},
	author = {Xie, Shaoan and Zhang, Zhifei and Lin, Zhe and Hinz, Tobias and Zhang, Kun},
	month = dec,
	year = {2022},
	note = {arXiv:2212.05034 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/DPMTNX3Z/Xie et al. - 2022 - SmartBrush Text and Shape Guided Object Inpaintin.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/664B6J7X/2212.html:text/html},
}

@misc{zhang_sine_2022,
	title = {{SINE}: {SINgle} {Image} {Editing} with {Text}-to-{Image} {Diffusion} {Models}},
	shorttitle = {{SINE}},
	url = {http://arxiv.org/abs/2212.04489},
	
	urldate = {2022-12-21},
	publisher = {arXiv},
	author = {Zhang, Zhixing and Han, Ligong and Ghosh, Arnab and Metaxas, Dimitris and Ren, Jian},
	month = dec,
	year = {2022},
	note = {arXiv:2212.04489 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/DJIT7325/Zhang et al. - 2022 - SINE SINgle Image Editing with Text-to-Image Diff.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/68KV8TQ9/2212.html:text/html},
}

@misc{wallace_edict_2022,
	title = {{EDICT}: {Exact} {Diffusion} {Inversion} via {Coupled} {Transformations}},
	shorttitle = {{EDICT}},
	url = {http://arxiv.org/abs/2211.12446},
	doi = {10.48550/arXiv.2211.12446},
	
	urldate = {2022-12-22},
	publisher = {arXiv},
	author = {Wallace, Bram and Gokul, Akash and Naik, Nikhil},
	month = nov,
	year = {2022},
	note = {arXiv:2211.12446 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/YKX5RUY5/Wallace et al. - 2022 - EDICT Exact Diffusion Inversion via Coupled Trans.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/ZMG6JG8N/2211.html:text/html},
}

@misc{kwon_diffusion_2022,
	title = {Diffusion {Models} already have a {Semantic} {Latent} {Space}},
	url = {http://arxiv.org/abs/2210.10960},
	
	urldate = {2023-01-26},
	publisher = {arXiv},
	author = {Kwon, Mingi and Jeong, Jaeseok and Uh, Youngjung},
	month = oct,
	year = {2022},
	note = {arXiv:2210.10960 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/X64C2FJQ/Kwon et al. - 2022 - Diffusion Models already have a Semantic Latent Sp.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/CISHMBID/2210.html:text/html},
}

@misc{avrahami_spatext_2022,
	title = {{SpaText}: {Spatio}-{Textual} {Representation} for {Controllable} {Image} {Generation}},
	shorttitle = {{SpaText}},
	url = {http://arxiv.org/abs/2211.14305},
	doi = {10.48550/arXiv.2211.14305},
	urldate = {2023-01-28},
	publisher = {arXiv},
	author = {Avrahami, Omri and Hayes, Thomas and Gafni, Oran and Gupta, Sonal and Taigman, Yaniv and Parikh, Devi and Lischinski, Dani and Fried, Ohad and Yin, Xi},
	month = nov,
	year = {2022},
	note = {arXiv:2211.14305 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Graphics, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/RLTNCAMQ/Avrahami et al. - 2022 - SpaText Spatio-Textual Representation for Control.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/RC4VH3R4/2211.html:text/html},
}

@misc{chen_importance_2023,
	title = {On the {Importance} of {Noise} {Scheduling} for {Diffusion} {Models}},
	url = {http://arxiv.org/abs/2301.10972},
	
	urldate = {2023-01-28},
	publisher = {arXiv},
	author = {Chen, Ting},
	month = jan,
	year = {2023},
	note = {arXiv:2301.10972 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Graphics, Computer Science - Machine Learning, Computer Science - Multimedia},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/KCBJV8MY/Chen - 2023 - On the Importance of Noise Scheduling for Diffusio.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/THV2NCZS/2301.html:text/html},
}

@misc{ramesh_hierarchical_2022,
	title = {Hierarchical {Text}-{Conditional} {Image} {Generation} with {CLIP} {Latents}},
	url = {http://arxiv.org/abs/2204.06125},
	urldate = {2023-01-28},
	publisher = {arXiv},
	author = {Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
	month = apr,
	year = {2022},
	note = {arXiv:2204.06125 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
	file = {arXiv Fulltext PDF:/Users/viditgeol/Zotero/storage/TXNV35NL/Ramesh et al. - 2022 - Hierarchical Text-Conditional Image Generation wit.pdf:application/pdf;arXiv.org Snapshot:/Users/viditgeol/Zotero/storage/XGXXHDL6/2204.html:text/html},
}


@inproceedings{gafni2022make,
  title={Make-a-scene: Scene-based text-to-image generation with human priors},
  author={Gafni, Oran and Polyak, Adam and Ashual, Oron and Sheynin, Shelly and Parikh, Devi and Taigman, Yaniv},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part XV},
  pages={89--106},
  year={2022},
  organization={Springer}
}

@article{wu2022uncovering,
  title={Uncovering the Disentanglement Capability in Text-to-Image Diffusion Models},
  author={Wu, Qiucheng and Liu, Yujian and Zhao, Handong and Kale, Ajinkya and Bui, Trung and Yu, Tong and Lin, Zhe and Zhang, Yang and Chang, Shiyu},
  journal={arXiv preprint arXiv:2212.08698},
  year={2022}
}


@inproceedings{sohl2015deep,
  title={Deep unsupervised learning using nonequilibrium thermodynamics},
  author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle={International Conference on Machine Learning},
  pages={2256--2265},
  year={2015},
  organization={PMLR}
}

@article{song2020denoising,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv preprint arXiv:2010.02502},
  year={2020}
}
@article{salimans2022progressive,
  title={Progressive distillation for fast sampling of diffusion models},
  author={Salimans, Tim and Ho, Jonathan},
  journal={arXiv preprint arXiv:2202.00512},
  year={2022}
}
@article{feng2022training,
  title={Training-Free Structured Diffusion Guidance for Compositional Text-to-Image Synthesis},
  author={Feng, Weixi and He, Xuehai and Fu, Tsu-Jui and Jampani, Varun and Akula, Arjun and Narayana, Pradyumna and Basu, Sugato and Wang, Xin Eric and Wang, William Yang},
  journal={arXiv preprint arXiv:2212.05032},
  year={2022}
}

@inproceedings{huang2023collaborative,
  title={Collaborative diffusion for multi-modal face generation and editing},
  author={Huang, Ziqi and Chan, Kelvin CK and Jiang, Yuming and Liu, Ziwei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6080--6090},
  year={2023}
}

@article{cao2023masactrl,
  title={MasaCtrl: Tuning-Free Mutual Self-Attention Control for Consistent Image Synthesis and Editing},
  author={Cao, Mingdeng and Wang, Xintao and Qi, Zhongang and Shan, Ying and Qie, Xiaohu and Zheng, Yinqiang},
  journal={arXiv preprint arXiv:2304.08465},
  year={2023}
}

@article{patashnik2023localizing,
  title={Localizing Object-level Shape Variations with Text-to-Image Diffusion Models},
  author={Patashnik, Or and Garibi, Daniel and Azuri, Idan and Averbuch-Elor, Hadar and Cohen-Or, Daniel},
  journal={arXiv preprint arXiv:2303.11306},
  year={2023}
}

@article{mou2023t2i,
  title={T2i-adapter: Learning adapters to dig out more controllable ability for text-to-image diffusion models},
  author={Mou, Chong and Wang, Xintao and Xie, Liangbin and Zhang, Jian and Qi, Zhongang and Shan, Ying and Qie, Xiaohu},
  journal={arXiv preprint arXiv:2302.08453},
  year={2023}
}
@inproceedings{yang2023paint,
  title={Paint by example: Exemplar-based image editing with diffusion models},
  author={Yang, Binxin and Gu, Shuyang and Zhang, Bo and Zhang, Ting and Chen, Xuejin and Sun, Xiaoyan and Chen, Dong and Wen, Fang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={18381--18391},
  year={2023}
}

@article{mou2023dragondiffusion,
  title={DragonDiffusion: Enabling Drag-style Manipulation on Diffusion Models},
  author={Mou, Chong and Wang, Xintao and Song, Jiechong and Shan, Ying and Zhang, Jian},
  journal={arXiv preprint arXiv:2307.02421},
  year={2023}
}

@article{epstein2023diffusion,
  title={Diffusion self-guidance for controllable image generation},
  author={Epstein, Dave and Jabri, Allan and Poole, Ben and Efros, Alexei A and Holynski, Aleksander},
  journal={arXiv preprint arXiv:2306.00986},
  year={2023}
}

@article{hachnochi2023cross,
  title={Cross-domain Compositing with Pretrained Diffusion Models},
  author={Hachnochi, Roy and Zhao, Mingrui and Orzech, Nadav and Gal, Rinon and Mahdavi-Amiri, Ali and Cohen-Or, Daniel and Bermano, Amit Haim},
  journal={arXiv preprint arXiv:2302.10167},
  year={2023}
}
@article{oquab2023dinov2,
  title={Dinov2: Learning robust visual features without supervision},
  author={Oquab, Maxime and Darcet, Timoth{\'e}e and Moutakanni, Th{\'e}o and Vo, Huy and Szafraniec, Marc and Khalidov, Vasil and Fernandez, Pierre and Haziza, Daniel and Massa, Francisco and El-Nouby, Alaaeldin and others},
  journal={arXiv preprint arXiv:2304.07193},
  year={2023}
}
@article{raghu2021vision,
  title={Do vision transformers see like convolutional neural networks?},
  author={Raghu, Maithra and Unterthiner, Thomas and Kornblith, Simon and Zhang, Chiyuan and Dosovitskiy, Alexey},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={12116--12128},
  year={2021}
}
@article{walton2022stylenat,
  title={StyleNAT: Giving each head a new perspective},
  author={Walton, Steven and Hassani, Ali and Xu, Xingqian and Wang, Zhangyang and Shi, Humphrey},
  journal={arXiv preprint arXiv:2211.05770},
  year={2022}
}

@inproceedings{bansal2023universal,
  title={Universal guidance for diffusion models},
  author={Bansal, Arpit and Chu, Hong-Min and Schwarzschild, Avi and Sengupta, Soumyadip and Goldblum, Micah and Geiping, Jonas and Goldstein, Tom},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={843--852},
  year={2023}
}
@article{song2020score,
  title={Score-based generative modeling through stochastic differential equations},
  author={Song, Yang and Sohl-Dickstein, Jascha and Kingma, Diederik P and Kumar, Abhishek and Ermon, Stefano and Poole, Ben},
  journal={arXiv preprint arXiv:2011.13456},
  year={2020}
}

@article{xu2023prompt,
  title={Prompt-Free Diffusion: Taking" Text" out of Text-to-Image Diffusion Models},
  author={Xu, Xingqian and Guo, Jiayi and Wang, Zhangyang and Huang, Gao and Essa, Irfan and Shi, Humphrey},
  journal={arXiv preprint arXiv:2305.16223},
  year={2023}
}
@inproceedings{zhang2018unreasonable,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={586--595},
  year={2018}
}
@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part V 13},
  pages={740--755},
  year={2014},
  organization={Springer}
}


@article{faceparse,
  title={https://github.com/zllrunning/face-parsing.PyTorch},
  author={zllrunning},
    year={2019},
journal={github},
  publisher={github}
}

==> tables/struct.tex <==
\begin{table}
\centering
\caption{Quantitative results for structure control on CelebA-HQ validation dataset.}
\vspace{-1.em}
\begin{tabular}{ccccc}
\toprule
Method & SEAN [14]  & SAP  \\ 
\midrule
 mIoU ($\uparrow$)/SSIM ($\uparrow$) & 0.64 / 0.32 & \textbf{0.67 / 0.52} \\
\bottomrule
\end{tabular}
\label{tab:exp_iou}
\vspace{-2em}
\end{table}
